Yoga Pose Classification Using Transfer Learning

Yoga has recently become an essential aspect of human existence for maintaining a healthy body and mind. People find it tough to devote time to the gym for workouts as their lives get more hectic and they work from home. This kind of human pose estimation is one of the notable problems as it has to deal with locating body key points or joints. Yoga-82, a benchmark dataset for large-scale yoga pose recognition with 82 classes, has challenging positions that could make precise annotations impossible. We have used VGG-16, ResNet-50, ResNet-101, and DenseNet-121 and finetuned them in different ways to get better results. We also used Neural Architecture Search to add more layers on top of this pre-trained architecture. The experimental result shows the best performance of DenseNet-121 having the top-1 accuracy of 85% and top-5 accuracy of 96% outperforming the current state-of-the-art result.

==> referencesbib <==
@misc{omalley2019kerastuner,
    title        = {KerasTuner},
    author       = {O'Malley, Tom and Bursztein, Elie and Long, James and Chollet, Fran\c{c}ois and Jin, Haifeng and Invernizzi, Luca and others},
    year         = 2019,
    howpublished = {\url{https://github.com/keras-team/keras-tuner}}
}

@inproceedings{1_verma2020yoga,
  title={Yoga-82: a new dataset for fine-grained classification of human poses},
  author={Verma, Manisha and Kumawat, Sudhakar and Nakashima, Yuta and Raman, Shanmuganathan},
  booktitle={Proceedings of the IEEE/CVF conference on computer vision and pattern recognition workshops},
  pages={1038--1039},
  year={2020}
}

@article{2_chen2020monocular,
  title={Monocular human pose estimation: A survey of deep learning-based methods},
  author={Chen, Yucheng and Tian, Yingli and He, Mingyi},
  journal={Computer Vision and Image Understanding},
  volume={192},
  pages={102897},
  year={2020},
  publisher={Elsevier}
}


@article{3_faisal2019monitoring,
  title={Monitoring methods of human body joints: State-of-the-art and research challenges},
  author={Faisal, Abu Ilius and Majumder, Sumit and Mondal, Tapas and Cowan, David and Naseh, Sasan and Deen, M Jamal},
  journal={Sensors},
  volume={19},
  number={11},
  pages={2629},
  year={2019},
  publisher={MDPI}
}

@inproceedings{4_boualia2019pose,
  title={Pose-based human activity recognition: a review},
  author={Boualia, Sameh Neili and Amara, Najoua Essoukri Ben},
  booktitle={2019 15th international wireless communications \& mobile computing conference (IWCMC)},
  pages={1468--1475},
  year={2019},
  organization={IEEE}
}

@inproceedings{5_chowdhury2020hactnet,
  title={hActNET: an improved neural network based method in recognizing human activities},
  author={Chowdhury, Atiqul Islam and Ashraf, Mohsena and Islam, Ashraful and Ahmed, Eshtiak and Jaman, Md Saroar and Rahman, Mohammad Masudur},
  booktitle={2020 4th international symposium on multidisciplinary studies and innovative technologies (ISMSIT)},
  pages={1--6},
  year={2020},
  organization={IEEE}
}


@article{6_nagalakshmi2021analysis,
  title={The analysis of the impact of yoga on healthcare and conventional strategies for human pose recognition},
  author={Nagalakshmi Vallabhaneni, Dr P Prabhavathy},
  journal={Turkish Journal of Computer and Mathematics Education (TURCOMAT)},
  volume={12},
  number={6},
  pages={1772--1783},
  year={2021}
}

@inproceedings{7_agrawal2020implementation,
  title={Implementation of machine learning technique for identification of yoga poses},
  author={Agrawal, Yash and Shah, Yash and Sharma, Abhishek},
  booktitle={2020 IEEE 9th international conference on communication systems and network technologies (CSNT)},
  pages={40--43},
  year={2020},
  organization={IEEE}
}

@ARTICLE{8_9343347,
  author={Liaqat, Sidrah and Dashtipour, Kia and Arshad, Kamran and Assaleh, Khaled and Ramzan, Naeem},
  journal={IEEE Sensors Journal}, 
  title={A Hybrid Posture Detection Framework: Integrating Machine Learning and Deep Neural Networks}, 
  year={2021},
  volume={21},
  number={7},
  pages={9515-9522},
  doi={10.1109/JSEN.2021.3055898}}

@book{9_kumar2020yoga,
  title={Yoga pose detection and classification using deep learning},
  author={Kumar, Deepak and Sinha, Anurag},
  year={2020},
  publisher={LAP LAMBERT Academic Publishing}
}


@article{10_kulikajevas2021detection,
  title={Detection of sitting posture using hierarchical image composition and deep learning},
  author={Kulikajevas, Audrius and Maskeliunas, Rytis and Dama{\v{s}}evi{\v{c}}ius, Robertas},
  journal={PeerJ computer science},
  volume={7},
  pages={e442},
  year={2021},
  publisher={PeerJ Inc.}
}

@article{11_panigrahy2021detection,
  title={Detection of ventricular fibrillation rhythm by using boosted support vector machine with an optimal variable combination},
  author={Panigrahy, D and Sahu, PK and Albu, Felix},
  journal={Computers \& Electrical Engineering},
  volume={91},
  pages={107035},
  year={2021},
  publisher={Elsevier}
}


@article{12_nagalakshmi2021classification,
  title={Classification of yoga asanas from a single image by learning the 3d view of human poses},
  author={Nagalakshmi, Chirumamilla and Mukherjee, Snehasis},
  journal={Digital Techniques for Heritage Presentation and Preservation},
  pages={37--49},
  year={2021},
  publisher={Springer}
}

@inproceedings{13_chen2018shpd,
  title={SHPD: Surveillance human pose dataset and performance evaluation for coarse-grained pose estimation},
  author={Chen, Qiuhui and Zhang, Chongyang and Liu, Weiwei and Wang, Dan},
  booktitle={2018 25th IEEE International Conference on Image Processing (ICIP)},
  pages={4088--4092},
  year={2018},
  organization={IEEE}
}

@article{14_holte2012human,
  title={Human pose estimation and activity recognition from multi-view videos: Comparative explorations of recent developments},
  author={Holte, Michael B and Tran, Cuong and Trivedi, Mohan M and Moeslund, Thomas B},
  journal={IEEE Journal of selected topics in signal processing},
  volume={6},
  number={5},
  pages={538--552},
  year={2012},
  publisher={IEEE}
}

@article{15_chasmai2022view,
  title={A View Independent Classification Framework for Yoga Postures},
  author={Chasmai, Mustafa and Das, Nirjhar and Bhardwaj, Aman and Garg, Rahul},
  journal={SN Computer Science},
  volume={3},
  number={6},
  pages={476},
  year={2022},
  publisher={Springer}
}


